Explaining Reinforcement Learning to Mere Mortals: An Empirical Study

We present a user study to investigate the impact of explanations on non-experts' understanding of reinforcement learning (RL) agents. We investigate both a common RL visualization, saliency maps (the focus of attention), and a more recent explanation type, reward-decomposition bars (predictions of future types of rewards). We designed a 124 participant, four-treatment experiment to compare participants' mental models of an RL agent in a simple Real-Time Strategy (RTS) game. Our results show that the combination of both saliency and reward bars were needed to achieve a statistically significant improvement in mental model score over the control. In addition, our qualitative analysis of the data reveals a number of effects for further study.

==> 0-TODO-List.tex <==


\begin{figure*}
\FIXME{
\textbf{\underline{Paper Information}}
\begin{enumerate}

    \item{All editable figures are located in our Google drive folder: IJCAI/Results (\url{https://drive.google.com/drive/folders/1wbzmx4L9ley608tyZIVpfs5_IlIQfKLV})   (SAVE THIS NOTE forever)}

    \item JED (future paper thoughts)): we have decided to shove the discussion of the difference in the ``grid'' saliency from the EVERYTHING treatment and the ``row'' saliency from the saliency treatment to the long form journal paper
    
    \item JED: (future paper thoughts)) Random seems to be a subclass of hard, but we know the reason for the difficulty--namely that AI's life was mostly expended, so many actions become equivalent as they all lead to death. I have expounded on the ``random'' category a bit in a FIXME in section 4. Perhaps this could be a way to tie the 2 sections together more.
   
    
\end{enumerate}
}
\FIXME{
\textbf{\underline{TODO list}}
\begin{enumerate}
    
    \item justify explanation types (R3-9) \hfill IN PROGRESS Introduction

    \item gamers distributed pseudo-randomly? (R2-4)\hfill IN PROGRESS Methodology
    
    
    \item Supplemental materials both gathered and linked (R2-2a) \hfill Need to figure out where to put the link in the doc
        \begin{enumerate}
            \item Data table of significance tests (R0-1) in progress
            \item More info about each DP (R1-3) done
            \item Questionnaires (R2-4a) done
            \item more stuff (source, scripts, etc) done
        \end{enumerate}

\end{enumerate}

}
\FIXME{
\textbf{\underline{DONE list}}
\begin{enumerate}
    \item Add error bars to Fig 8 (R1-4) \hfill DONE
    \item clarify inuition for soundndess and completeness for these expos (R3-10) \hfill DONE Introduction
    \item typo that we cant identify (R2-7)\hfill IGNORED
    \item Task prediction should be accompanied by confidence rating (R3-5) \hfill IGNORED
    \item demographic information (R3-6) \hfill IGNORED  
    
    \item Add other references from reviews (R2-10) \hfill Hoffman, Jaccard, Greydanus, Rosenfeld DONE
    
    
    \item Saliency that ``worked best'' is lame (R2-2) \hfill COMPLETE Background
   
    \item text in figure 1 too small (R2-8) \hfill COMPLETE figure 1 caption
   
    \item Justify choice of building game (R2-1) \hfill DONE Methodology
    \item clarify recruitment process, approved by IRB? (R2-3)\hfill COMPLETE Methodology

    \item Nasa TLX? (R2-5) \hfill IGNORE
    \item clarify DPs vs task (R3-2) \hfill DONE Methodology
    \item 20 min tutorial enough time to learn the agent? (R3-3)\hfill DONE Methodology
    \item compensation information (R3-7) \hfill DONE Methodology 
    \item How are tasks different? how were they chosen? (R3-4)\hfill DONE Methodology
    
    
    
    \item what coding method? (R3-1) \hfill DONE results 4
    \item Add reference to jaccard (R2-9) \hfill DONE results 4
    \item Clarify process of explanation/prediction (R1-1) \hfill DONE Methodology/results 5
    \item Discuss learning effects (R1-2) \hfill DONE Results 5
    
    

    
    
    \item what is the contribution/impact of this work (R2-6, R3-8) \hfill DONE Conclusion
    
    \item Cut Hughes \& Parkes\hfill DONE
\end{enumerate}

}

\end{figure*}

\begin{figure*}
\FIXME{
\textbf{\underline{Global Search}}
\begin{enumerate}



\item [DONE] by JED Sun Late - Remove \emph{ALL} mentions of ``better'' or ``worse'' UNLESS we have a p value and statistics to back it up.

\item [DONE] by JED Sun Late - Find the first place we mention DP and make sure it's spelled out Decision Point

\item [DONE] by JED Sun Late - Search for ``"'' (double quotes) in the source code. V2 made it harder to catch.

 \item [DONE] by JED Sun Late - MMB to anyone: global: I don't much like calling "Saw Rewards" a "treatment". Let's just stick with the 4 original treatments, and when we want to talk about people who saw rewards, do it in lower case when needed add on  ``(\treatment{Rewards} and \treatment{Everything})".  And likewise with "Saw Saliency".

\item [DONE] by JED Sun Late - ``expert'' refers ONLY to AI expertise.  If referring to game expertise, use ``gamer'' instead. 

\item [DONE] by JED Sun Late - DP acronym usage (it is shorter, do NOT write decision point more than around twice in the paper).


\item [DONE] by JED Sun Late - FIXME search and a ** search in the pdf.

\item [DONE] by JED Sun Late - Make sure every time we reference \textbf{treatments}, we capitalise them. control $\rightarrow$ Control, saliency $\rightarrow$ Saliency, etc.

\item [DONE] by JED Sun Late -  remove the word ``visual'' from explanations


\item [DONE] by JED Sun Late - participants are people ``participants who'' is better than ``participants that''



\item Be consistent about referring to the AI/Agent/Etc (we may need to decide which we want to use as a group)

\item Ensure that the quoting of participants is consistent.

\end{enumerate}
}
\end{figure*}

\begin{figure*}
\FIXME{
Draft Status Table

\footnotesize
\begin{tabular}{l|l|l|p{.4\linewidth}}
Section & Status & PageBudget & Notes\\
Abstract & D2 
& -
& 
\\
Introduction & D2.5 
& Title+ab+intro: 3/4P-ok
& Jed please read this section for edits
\\\hline

Background & D2 
& 1/2P ok :)
& 
\\
$\quad$ - (Rewards) & D2 
& 
& 
\\
$\quad$ - (Saliency) & D2 
& 
& 
\\\hline

Methodology & D2 
& 1P to 1.5P for now
& Read for cuts? and edits
\\
$\quad$ - (Participants) & D2 
& 
& 
\\
$\quad$ - (Procedures) & D2 
& 
& 
\\
$\quad$ - (System Overview) & D2 
& 
& 
\\\hline

Results MM  & D2 
& 1.5P-ok
& Read for edits
\\
$\quad$ - (Is Everything Better?) & D2 
& 
& 
\\
$\quad$ - (Nuances) & D2 
& 
& 
\\
$\quad$ - (Discussion) & D2 
& 
& 
\\\hline

Results Pred  & D1 
& 2ishP-OKish but... 
&  Read for comprehension (NOT edits)
\\
$\quad$ - (Nothing is ok?) & D1 
& 
& 
\\
$\quad$ - (hard decisions) & D1 
& 
& 
\\
$\quad$ - (End of task) & D1 
& 
& 
\\
$\quad$ - (Overwhelm) & D1 
& 
& 
\\
$\quad$ - (Discussion) & D1 
& 
& 
\\\hline

Threats & D2 
& 1/4P-ok
& 
\\

Conclusion & D2.25 
& 1/4P 
& 
\\

Bibliography & D3 
& 1P-ok
& 
\end{tabular}
}
\end{figure*}

\setcounter{page}{0}

==> 6-Discussion.tex <==
\section{Discussion}

\FIXME{High level:\\
Challenges of the study\\
Point out 100\% is not the goal of the study. We don't want our explanation to get the people to 100\%, but rather just who did better.\\
Not a ton of time for prediction, RTS time constraints\\
AAA @ MMB: JED \& I both think that we do a fair amount of discussion in the results sections themselves. We can pull all the information together in the conclusion, so we think that we can safely get rid of the discussion section. Below is my stab, and it's all I think we can say in the discussion.}

\boldify{For example, the final mental model was good because it allowed participants to describe more holistically the AI's reasoning}

With the final evaluation, the participants had to provide a ``rulebook'' of the AI, its process to make decisions \emph{generally}.
This provided a global interpretation of the agent, and the results indicated that users should have access to \emph{both} saliency + decomposed rewards to understand it more holistically.


\boldify{However, providing a ``Rulebook'' of the AI is very difficult, since they could accidentally omit information}

However, providing a rulebook is hard;
for example, the participants might have accidentally omitted information or forgotten something from an early DP.
This means that the participants needed a more concrete way to test their knowledge.

\boldify{This is why prediction is used, which allows participants to ``test'' their knowledge in a more concrete setting}

Prediction clicks allowed them this opportunity, where they had a chance to test their understanding of the AI within the context of the simulator.
These results varied wildly, and they seemed to oppose the result that the user should have everything, since the \treatment{Everything} participants, more often than not, did \emph{not} perform best at each DP.

\boldify{However, to avoid human fatigue, participants could only see 14 decision points, limiting the amount of data}

However, to limit the effect of human fatigue, the participants were restricted to $\approx 2$ hours to complete the study.
This meant that the number of decisions that a participant could see was limited to 17 (3 in the tutorial and 14 in the study).



==> a-leftovers.tex <==
\section{Methodology}
\FIXME{Participants, Procedures, How do we evaluate, Treatments}

\subsection{Participant Demographics}
\boldify{We recruited participants from a survey distributed around Our University and online, and we received over 200 responses}
\\
\boldify{We rejected participants that might have pre-existing knowledge on how AI works, since they wouldn't need to rely on the explanations for understanding.}
\\
\boldify{We decided to exclude Computer Science (CS) majors and Electrical \& Computer Engineering (ECE) majors once they had been vetted to have not had any artificial intelligence classes}
\\
\boldify{We ran a total 124 participants in our study, and the breakdown of their college majors is in table [1].}
\\
\subsection{Procedures}

\boldify{We scheduled around participant availability in sessions that ran from as few as 1 participant to as many as 6 participants per session, running a total of 55 sessions}
\\
\boldify{To ensure that the participants experienced approximately the same amount of stresses from classes etc, we completed our study within a month of the term's beginning}
\\
\boldify{Since none of the participants had seen this game before, and we didn't require RTS experience for the study, we tutorialized the game for the first while of the study to ensure that we could call them ``domain experts'' such as in Penney et al.'s study}
\\
\boldify{To make sure participants were focused on the explanations and not being engrossed in the game, we simplified the Real-Time Strategy (RTS) game to a series of sequential decisions, an example of which can be seen in Figure [1].}
\\
\boldify{At each of the decision points, participants followed the following workflow:\\1)Predict the action that the AI will take at this decision point (explanation invisible), and tell us why you think this is the action\\2)See if you were wrong or right (explanation visible) and use the information provided to validate your correctness or learn why you were incorrect.\\3)Can you see a flaw in the AI's reasoning? (explanation visible)\\4)What would you ask the system, if anything?}
\\
\boldify{We wanted them to predict the AI's action to see if these explanations provided information that would allow them to accurately understand the AI}
\\
\boldify{We asked questions (specific to a treatment) in order to understand what information they were receiving from the explanations, and the questions can be seen in table [2] AAA - I made sketches of the tables.}
\\
\boldify{The participants saw 14 decision points total, each one asking the questions in Table [2].}
\\
\boldify{After the final decision point, the participants were asked the question to describe the steps or method that the AI took towards its decision making, which can be seen in figure [2].}
\\
\boldify{Every action they took and answer they gave was logged, and the system generated a text file that we could analyze}
\\
\boldify{After they had answered the final question on their screen, the participants were asked to fill out a post-task questionnaire that asked what was helpful about the information given to them, what was problematic about the information given to them, in which circumstances the AI will make a bad decision, as well as the NASA Task Load indeX (TLX) to help us measure how cognitively taxing the task was.}
\\
\boldify{During sandboxing, we discovered that we were getting responses to the ``helpful'' and ``problematic'' questions that did not directly address the \emph{explanations}, but rather the tutorial and/or cheat sheet.}
\\
\boldify{We changed the questions per treatment to be more directed at the explanations, and these questions can be seen in table [3].}
\\
\subsection{Treatment}

\subsubsection{How do we define an explanation}

\\.

\boldify{We define an explanation as a tuple Explanation = < Artifacts, Behaviors, Score>, where Artifacts $\in$ \{Saliency, Rewards, Saliency + Rewards\}, Behaviors are considered the feedback received from clicking on any of the above, and score is the displayed point value to the left of the game map. }
\\.

\subsubsection{Control}

\input{figure/Prediction(1).tex}

\subsubsection{Saliency Treatment}

\\.

\boldify{The saliency treatment saw the saliency maps for the \emph{most positive} or \emph{least negative} total reward bar, for example in Figure ~\ref{fig:controlInterface}.}

\\.

\boldify{We made this experiment design decision to prevent our participants in this treatment from learning too much about the other type of information, i.e. the reward bars, we restricted it to the action that was taken, seen in Figure [4].}

\subsubsection{Rewards Treatment}

\\.

\boldify{The rewards treatment saw \emph{all} rewards for all possible actions, such as in Figure [4]. Not only can they see the action that was taken, like in Attack Q\_ in Figure [4], but they can also see the actions that were \emph{not} taken}

\\.

\boldify{We made this experiment design decision to see if participants would choose a bar that is in line with the AI's reasoning, such as Attack Q\_ in Figure [4], or if the participants would choose a bar such as Attack Q\_, where they think that the AI is just terrified of large negative penalty. AAA - I'm trying to get at the fear of punishment or the glutton for reward}

\subsubsection{Saliency, Rewards, and everything else}

\\.

\boldify{We designed the Saliency, Rewards, and Everything Else treatment, which we will just call ``The Everything Treatment'', to see if our participants needed everything to gain the most information out of the system}

\\.

\boldify{We made the experiment design decision to show the saliency maps for a \emph{selected} reward bar, such as the red connecting arrow in Figure [5]}

\\.

\boldify{We made this decision to be as truthful to the internal reasoning of the AI as we could, even though it may have impacted people's perceptions of the explanations that they saw}



\\.

\boldify{We designed the control to be representative of how things are done in current RTS games, where the viewer has little-to-no explanation as to why an actor performed some action}

\\.

\boldify{We asked the participants very similar questions to the other treatments, without revealing too much about the inner-workings of the system.}

\\.

\boldify{Figure [6] shows the control screen, which essentially boils down to just viewing the game map.}

\subsection{How we evaluated}

\boldify{To answer which combination of the treatments performed the best, we extracted the participants' predictions from the logged information, and we compared them against what the AI actually did}
\\
\boldify{If the participant clicked on the object that the AI attacked at that decision point, we marked their answer as correct. Otherwise, we marked them as incorrect.}
\\
\boldify{Since the participant had to \emph{justify why} they clicked on an object, we gained insight into their reasoning through affinity diagramming.... AAA - Let's talk about this on 11/29/2018. I think there's something to be said here.}
\\
\boldify{In order to help us understand what the participants thought was helpful or problematic about the explanation given to them, we affinity diagrammed the responses to generate 2 sets of codes for ``helpful'' and ``problematic'' information.}
\\
\boldify{Two researchers reached an agreement of X\% over 20\% of the corpus, and then both corpora were coded by one of the researchers.}
\\
\boldify{To answer what information demand was satisfied by each explanation, two researchers familiar with the Lim \& Dey Intelligibility Types looked at the participants' responses to the last question of each treatment: ``What, if anything, do you want to ask the AI at this point?''}
\\
\boldify{To make sure that each of the coders could code the data set accurately, an agreement test was performed on 20\% of the data. The coders reached Y\% agreement, above the minimum threshold set by AAA - Who should we cite for this?}
\\
\boldify{The rest of the data set was coded by one of the coders, and then the researchers met to discuss the graphs generated, discussed in section 5.}
\\


\FIXME{AAA - I'm not so sure that Newn's work might be a fit here. I think I'm making too much of a stretch.\\
\boldify{Humans are really good at following the gaze of another entity and inferring intentions from it ~\cite{FIXME Cite Newn et al.'s work} }\\

Newn et al. studied how humans use gaze tracking~\cite{newn2016exploring}, and they discovered that people are exceptional at following someone's gaze and understanding why they're looking at an object.

\boldify{We wanted to see if this ability transferred to a non-living entity, so participants in the saliency treatment saw where the ``eyeballs'' of the AI fell, which they could see in region 3}

We then wondered if saliency maps allowed participants to ``follow the AI's gaze'' and help them understand \emph{why} the AI made particular decisions from what it was looking at.
}

\boldify{One of the issues that might have arisen was the choice to perform an in-lab study or to deploy the system on mechanical turk}

Why choose to have an in-lab study, rather than deploy the system on mechanical turk?
Each of these methods have their strengths and weaknesses for data collection.

\boldify{Mechanical turk has the advantage that we might have been able to gather much more data, but we couldn't have controlled for \emph{life}, where there might have been people just taking random guesses at the prediction task}

Mechanical turk allows the collection of vast amounts of data.
However, the ability to control negative impacts on the data is lost.
For example, participants are more likely to randomly guess during the prediction task or provide quick answers in the final description just to get paid.



Potentially discussion. Jon and I discussed removing it in favour of citing the book on his desk.

\boldify{An in-lab study allowed us to negate this by controlling the environment that the participants were in, free from the distractions of screaming children or anything else that life throws at them}

In-lab studies negate a lot of these concerns, since the environment that the participants experienced the system in is controlled.
For example, the participants couldn't check their phones while in the lab, so they were more focused on the system.
However, this meant that the amount of data collected was smaller, but the quality drastically improved~\cite{FIXME - Probably need some source on this}.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%HERE LIES THE OLD METHODOLOGY SECTION THAT JED REPLACED, may it rest in peace...

%\boldify{We recruited participants from a survey distributed around Our University and online, and we received over 200 responses}

%We wanted each participant to be someone who might benefit from the explanations, not someone who could deduce the system internals without explanation.
%This meant excluding those with exposure to AI principles.
To accomplish this, we excluded all Computer Science majors and anyone who had taken an AI course.
Information about AI exposure was included in the survey we distributed at \redact{Oregon State University}.

\boldify{We decided to exclude Computer Science (CS) majors and Electrical \& Computer Engineering (ECE) majors once they had been vetted to have not had any artificial intelligence classes}

\boldify{We ran a total 124 participants in our study, and the breakdown of their college majors is in Table~\ref{table:participants}.}

We received over 200 survey responses, and we found 124 participants that met our criteria and participated in the study.
39 majors were represented in our study.
We defined RTS expertise as having at least 10 hours of experience with any of these games, and 78\% of our participants fit this criteria.
Table~\ref{table:participants} shows the breakdown of participant demographics.

\subsection{Procedures}

\FIXME{JED: this ection needs to be bolstered with a clearer description of the task (need to define DP here someplace). 
Its also very long winded in places that it doesnt need to be, e.g. we didnt plan for ``similar levels of academic'' stress at all, and even if we did, that is not important enough to spend characters on in a 6 page document.}

\boldify{We scheduled around participant availability, in sessions that ran from as few as 1 participant to as many as 6 participants per session, where everyone had their own workstation; we ran a total of 55 sessions.}

%\FIXME{ OLD VERSION AAA - We offered multiple sessions a day, every day of the week.
%We wanted to make sure that when a participant was available, we had a session that they could have, even if they were the only one.
%We ran a total of 55 sessions within the first month of the term, running as little as 1 to as many as 6 participants per session.
%We randomly assigned each participant group a treatment right before they entered the lab, where they worked at their individual workstations for about 2 hours at a time.}

To increase the chances that we could quickly schedule participants, we offered multiple sessions a day, every day of the week.
We ran a total of 55 sessions, running between 1 and 6 participants in each session.
Each session was randomly assigned a treatment, using a random number generator.
We timed the study between September and October, 2018, hoping that participants had similar levels of academic stress.

\boldify{We wanted participants focused on the explanations, so we had to be sure that they didn't get engrossed in something as complex as a full Real-Time Strategy (RTS) game, like in~\ref{fig:StarCraft2}}

Figure~\ref{fig:StarCraft2} shows an example of a common Real-Time Strategy game.
This game's rich visuals convey significant amount of activity and information.
For our study design, we wanted a smaller action space to reduce the chance that participants miss the action we were trying to explain, like what happened in~\cite{penney2018}'s study.


Our game used a small number of simple shapes to convey the game state and action.
Participants would replay a game played prior by an AI, where each game consisted of the AI making a short sequence of decisions.
Each decision was to choose which quadrant of the game map to attack.
We hoped the simple visuals and lack of extraneous detail would enable better focus on our explanations.
An example of our game can be seen in Figure~\ref{fig:sequentialDecisions}.



\boldify{This game was created in-house at our university because there are not as many sequential decision making games that we could easily interface with and change. The list of possible objects in the game that the participants saw can be seen in Figure~\ref{fig:TableOfObjects}}

We designed and built the game in-house to give us maximum flexibility and control in the game design, how our explanations would be rendered, and how our study questions could be integrated into the game.
During piloting, we could quickly change any aspect of the interface to make it more usable.
%the colors used in explanations, colors of objects on the game map, what shapes the objects were, and any other changes that needed to be made to the game or interface.
The game objects in the study are in Figure~\ref{fig:TableOfObjects}.

%Since we wanted a game that we could easily change components of, as well as being able to easily observe the user's interaction to the game through replay files, we created the sequential decision making game in-house at our university, which can be seen in Figure~\ref{fig:sequentialDecisions}.
%This allowed us to make changes quickly such as how the colors of the explanations looked, the colors of objects on the game map, what shapes the objects were, and any other changes that needed to be made to the game or interface during piloting.
%We have provided the list of objects that participants saw during the study in Figure~\ref{fig:TableOfObjects}.

%To look at the list of objects that the participants saw during the study, they are given in Figure~\ref{fig:TableOfObjects}. <-- AAA this was a teaching moment on passive voice for TM's benefit.

%\input{tables/questionTable.tex}


\boldify{Since none of our participants had seen this game before, we tutorialized the game for the first while of each session to ensure that we could call them ``domain experts'', similar to Penney et al.}

A researcher explained the game in a tutorial at the beginning of each study session to let participants become ``domain experts'' (similar to ~\cite{penney2018}'s study in StarCraft II).
This would allow participants to spend more time on explanation evaluation and less on making sense of the game.


%Because the game is created in-house and was never shown to the participants until they came into the lab, 1 of 2 researchers explained the game in a tutorial at the beginning of the session.
%This was to try to ensure that the participants in our study spent less time focused on making sense of the game and more time making sense of the explanations. 
%In fact, we wanted our participants to be so good that they could be considered ``domain experts'', similar to Penney et al.'s study in StarCraft II~\cite{penney2018}.

\input{figure/StarCraftII.tex}


\subsection{Technical Methodology}

\subsubsection{Our Implemented Decomposed Rewards}

\boldify{ Different events in the game are assigned a component or type based on their source and context. 
For instance, taking damage from an enemy may yield a small negative reward named "Took Damage" equal to the damage taken. 
This allows us to narrow down what sort of action the agent may have been seeking out or avoiding in a given decision.}



Reward decomposition bars assign context and types to different events, making an environment's total reward.
Our AI learned a positive/negative reward for damaging objects, and it also learned a destruction bonus/penalty, depending on if it's a friend or an enemy.
For example, if it hurts a friendly object, it loses 10 points for damage, but if it hurts an enemy, it gains 10 points for damaging it.

\boldify{
(NB could mention we use experience replay and dual networks).}

We trained a SARSA network to predict Q-values for these rewards, such that the sum of the reward types was the total reward ($\epsilon$-Q-values) for each action.
All of this information was presented to the participants as an explanation.

%We displayed these values as explanations to the user via a bar chart, showing the relative values for each action at a given decision. 
%We also have ``total" bars behind each group to communicate to the user what the total predicted Q value was, as that's the value used to make the decision.
%AAA - This last paragraph felt redundany


\FIXME{It'd be good to have some reference to an image of the relevant part of the interface here\\
AAA @ ZJ - We do, just above.}

\subsubsection{Our Implemented Saliency}
%\FIXME{OLD VERSION AAA - The input to the network was in the form of 7, 40x40 greyscale image layers namely HP, enemy tank, small forts, big forts, towns, cities, friend and enemy. 
%Then we found the pixels for each object in each layer. 
%Starting with the HP, we perturbed the HP of each object, noted the output for each output class and reward type, and subtracted that from the corresponding original un-perturbed image output.
%We noted this difference and inserted this value in the corresponding object's pixels in the HP Saliency Map for the corresponding output class and reward type. 
%Similarly, the enemy tank if present, was perturbed, and the difference between the perturbed image output and the unperturbed image output was inserted into the coordinates of the tank in the tank saliency map. 
%For the Size saliency map, for each object on the map, we zeroed out the pixels, and turned its pixels to 1 in its contrasting size layer. For example, for a small fort in the top right quadrant, we zero out its pixels in the small forts layer, and turn the pixels of its coordinates to 1 in the big forts layer. We toggled between small and big forts, and towns and cities. 
%Our approach to the City/Fort is similar to the Size saliency map except we toggled between the types. So small forts and towns were switched, and big forts and cities were switched. 
%The Friend/Enemy saliency map has the same approach as the previous two except here we switched the objects between the friend and enemy layers. }

\boldify{Our neural net was fed 7 greyscale image layers, and here are their names.}

The network took 7, 40x40 greyscale image layers namely HP, enemy tank, small forts, big forts, towns, cities, friend and enemy. We found the pixel coordinates for each object in each layer and proceeded to apply the perturbation method to generate saliency. 
The approach was to generate outputs by giving the true data and subtracting them from outputs generated by feeding in data that was changed by a small amount.  A large difference in those outputs would mean the system was more sensitive to that input.  This would suggest that the input was more important to the system. 

\boldify{Here is how our perturbation method works}
\FIXME{ OLD VERSION AAA - Starting with the HP, we perturbed the HP of each object, noted the output for each output class and reward type, and subtracted that from the corresponding original un-perturbed image output. We noted this difference and inserted this value in the corresponding object's pixels in the HP Saliency Map for the corresponding output class and reward type. 
Similarly, the enemy tank if present, was perturbed, and the difference between the perturbed image output and the unperturbed image output was inserted into the coordinates of the tank in the tank saliency map. }

Hp was real-valued, whereas all others were binary (there or not there), so we perturbed the HP of each object for each reward type and output class and subtracted that from the original un-perturbed image output.
This difference was inserted into the corresponding object's pixel coordinates in the corresponding saliency map.
Enemy tanks had a similar approach, but only switching between $1 \leftrightarrow 0$ in the layer.



For Size, each object on the map had its pixels zeroed out and turned to 1 in its opposing size layer.
Thus, a small fort in top-right quadrant would have its pixels zeroed out in the \textbf{small} fort layer.
Its pixels would then turn to 1 in the \textbf{big} forts layer.
These transformations changed $Small forts\leftrightarrow Big forts$ and $towns \leftrightarrow cities$.
An identical approach was taken for the City/Fort layer, where the transformations were $Forts \leftrightarrow Town/City$, depending on the size of the Fort.


\FIXME{OLD VERSION AAA - The Friend/Enemy saliency map has the same approach as the previous two except here we switched the pixel coordinates of objects between the friend and enemy objects and layers. }

The Friend/Enemy layer's transformations changed between $Friend \leftrightarrow Enemy$, except the pixel coordinates of objects switched between friend/enemy objects and layers.

\boldify{For the output, we combined some of the maps together, and we did this because....}
\FIXME{OLD VERSION AAA - The output saliency reflects five of the most pressing factors that would impact a neural network's decision. 
The saliency values are highly skewed, with the friend/enemy map usually having the highest values, thus being the most important to the network. 
It was a challenge, therefore, to choose an apt normalization method. 
We decided to globally normalize the saliency values. 
We ran the agent for 16000 episodes, and chose the maximum value for each map for each reward type and output class. 
We then used these values to normalize the respective map for that reward type and output class.}

In order to accurately reflect the AI's internal reasoning, we found a global normalization value for \emph{each} reward type and output class of attacking a quadrant by running 16000 episodes and choosing the max value for each saliency map.
We then normalized the 5 maps that reflect the most pressing factors impacting the network's decision.
This put every pixel's value $\in [0,1]$.
We took these values and colored them between [black, white].
As the pixels became more yellow, and eventually white, the more important they were.
These maps were presented to the participants of the \treatment{Saliency} and the \treatment{Everything} treatments, and the visualization was chosen to be consistent with prior research~\cite{newn2017evaluating}.

% Technical methodology goes here. I removed because it is not changing as much

\subsection{Treatment **D2**}

\subsubsection{How do we define an explanation}

\boldify{We define an explanation as a tuple Explanation = < Artifact, Behaviors, Score>, where Artifacts $\in$ \{Saliency, Rewards, Saliency + Rewards\}, Behaviors are considered the feedback received from clicking on any of the above, and score is the displayed point value to the left of the game map. }

$Explanation \rightarrow$ $<Artifacts, Behaviors, Score>$.
Artifacts are anything displayed to assist the participant in understanding the AI's behavior, the saliency maps and/or decomposed reward bars.
The Behavior is any feedback received from clicking on any artifact.
%, such as the overlay behavior in figure~\ref{**FIXME** Postage stamp sized image with the game map/overlay behavior}.
The Score is displayed beside the game map.

\FIXME{AAA - probably want an image (postage stamp size) showing the game map without \& with saliency overlay}

\input{figure/regionsUI}

\boldify{Figure~\ref{fig:userInterface} shows the different types of explanations that the participants saw, and Region 4 is constant across all treatments as the area that participants answered questions}

Figure~\ref{fig:userInterface} shows an example of what we showed participants, with highlighted regions.
The game map is in Region 1, where the AI acts out its choice.
The saliency maps are shown in Region 2.
Two treatments that gave saliency maps differed in their approach to showing saliency information to prevent revealing too much about the system, but their position on the interface was consistent.
Region 3 held the decomposed reward bars and total rewards for the 4 candidate actions.
The legend (upper right) used color to associate a reward bar with the type of reward it represented, including the gray bars for the sum total reward bars.
The wording was chosen to reinforce that these were predicted scores, not the actual score that the AI would receive.
Region 4 was where questions would be posed to all participants and where they could type their responses.
There were 4 treatments: \treatment{Control}, \treatment{Saliency}, \treatment{Rewards}, and \treatment{Everything}.

\subsubsection{Control}

\boldify{Region 1 in Figure~\ref{fig:userInterface} is the only region that the \treatment{Control} group saw. In their case, the explanation given to them was the game map being played, representative of how AI in RTS is handled currently}

The \treatment{Control} participants only saw the game map in Region 1.
No explanations were offered beyond what was visible in the game action, though the participants were free to rewind and re-watch any decision point.
The ability to rewind and watch decision points repeatedly is how current AI systems in this domain explain themselves.

\subsubsection{Saliency}

\boldify{The saliency treatment had access to regions 1 \& 2. However, Figure~\ref{FIXME- Need an example} shows the type of saliency that this treatment had access to.}

The \treatment{Saliency} participants saw both the game map and saliency maps.
The saliency maps conveyed which features of objects the AI is looking at when it makes a decision, so they know which input matters most.

\boldify{In order to avoid giving too much of the system away, we limited the participants' view of saliency to \emph{just} the action that was taken, so if the AI attacked Quadrant 1 (Q1), then we only showed the participants the saliency that was relevant to Q1.}

The \treatment{Saliency} treatment's saliency maps express information about what the AI was focusing on \emph{only} for the action selected, so the participants learned nothing about reward bars.
This maintained the study's integrity and abides by~\cite{kulesza2015principles}'s last principle about overwhelming.
%A more detailed approach was used in the ``Everything'' treatment, but the action-level granularity used here was chosen for 2 reasons.
%First, the more detailed approach exposes additional information about the AI's inner workings that we did not want exposed in this treatment.
%Second, showing this level of detail abides by Kulesza et al.'s last principle to not overwhelm the user~\cite{kulesza2015principles}.

\subsubsection{Rewards}
\boldify{Humans perform cost/benefit analysis all the time, even in the likes of their foraging behavior ~\cite{ FIXME any of the IFT work will do} }

Humans routinely perform cost/benefit analysis, trading off between expected rewards and time investment for those rewards.
This has been shown across a variety of domains from library card organization~\cite{pirolli1999information} to debugging tasks~\cite{piorkowski2015fix}.
The \treatment{Rewards} treatment showed predicted costs and benefits of taking actions.

\boldify{By phrasing the reward bars as a cost (bars below zero in Figure~\ref{fig:userInterface}, region 2)) and benefit (positive bars in that figure) prediction, we wanted to see if humans could infer these from the visual representation of \emph{why} the AI thought the way it did}

We wanted to see if the AI's thought process, or aspects of it, could be inferred by participants, since the decomposed reward bars were framed as a cost (bars $< 0$) and benefit(bars $> 0$) analysis from the AI.
Participants were shown both the decomposed reward bars (the thin ones) and the sum total (the gray ones) for each possible action.

\subsubsection{Saliency, Rewards, and everything else}
\boldify{The Saliency, Rewards, and Everything Else treatment, referred to as the ``Everything'' treatment, was a combination of the saliency maps and the reward bars, where each row of saliency corresponded with a decomposed reward bar}

The \treatment{Everything} treatment showed the participants all the explanation detail our system could provide.
The saliency maps corresponded to a particular predicted reward type for each action.
For example, the top row of saliency corresponded with a bar in Attack Q1, the second row corresponded to the same bar type in Attack Q2, and so on.
This level of detail was consistent with~\cite{kulesza2015principles}'s principle to be complete.

\subsection{Analysis Methods}

To answer RQ1, 2 researchers performed qualitative analysis on participant responses, iterating together to make a rule book for the code set.
They then independently coded 20\% of the data on these codes and reached $> 80\%$ agreement on those codes, consistent with the Jaccard index.
We provide details about this code set in the first Results sections.

To answer RQ2, we **FIXME TBD**

%Chunk taken from IUI 18
%How we did the coding
%How we moved from the qualitative coding to the score
%The scores for qualitative coding (IUI '19 before regression models) Effects without leaning on justifications.
%Less is better (5 or 6 sentences)
%For quantitative, we ran ANOVA on scores derived from scoring. Put the alpha in a footnote when we first use the p.

\FIXME{Notes for evaluation:\\
MMB: I like the idea someone wrote here: "just in time" in each Results section.\\
1) I think we want sub subsections for this, discussing how we analysed per results section.\\
2) For the prediction, we found out if they were right or wrong in their prediction.\\
%Insert a list of classifications, so we don't have to handwave and say ``trust me, this was objective''. Then we can say since this isn't objective, we just handled the counting and listing the type. NEVER USE THE WORD CODE! Dr. Burnett likes the word ``type''
}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% JED: Here are the pieces that were re-forged into the background section

\boldify{Traditionally, reinforcement learning agents are trained with a reward function that returns a single scalar value.
Accordingly, when agents learn Q-functions, which assign single scalar values to each action in a state.
Unfortunately, this only allows a very coarse comparison of the actions available in a state. 
In particular, we can compare the Q-value scales of those actions to see which is preferred by the agent. 
Such comparisons, however, don't provide insight into what trade-offs were involved ranking one action over another.}

Reinforcement learning agents learn scalar ``Q-functions'' through the network, assigning a value to each action in the action space.
The agents choose the largest of these total reward bars to determine which action to take.
However, they don't allow for \emph{why} the agent prefers one action over another.

\boldify{One approach to improving the ability to compare action values is to notice that rewards decompose into components, each representing a particular type of reward. For example, in a strategy game there may be reward types that measure the ``enemy damage taken" (negative reward), ``enemy damage given" (positive reward), and ``distance traveled" (negative reward). Often when designing a reinforcement learning environment, the concept of reward types is implicitly built into the designed reward function, but are not made explicit. In this work, we will make the reward types explicit by have the reward function return a reward decomposition vector at each step, rather than just a scalar.}

The total reward bars can be \emph{decomposed} into their positive/negative parts with a particular reward type, regaining the ability to distinguish preferences.
In a reinforcement learning environment, the reward types are implicitly built into the designed reward function;
however, our work builds on this approach by making the reward types explicit and returning a \emph{vector} of decomposed reward values.
\FIXME{AAA @ JED - I've tried to make this paragraph have some semblance of sense. Help plx}

\boldify{Recent work \cite{mugesh-ws18}, has shown how to learn from such decomposed reward functions, in a way that aims to achieve an optimal policy and also produce a decomposed Q-function $Q(s,a)$. The decomposed Q-function outputs a vector for each state-action pair, where the $i$'th component $Q_i(s,a)$ of the Q-vector gives the expected future cumulative reward for the $i$'th reward component. Given such a decomposed reward function it is now possible to compare the Q-vectors for two actions and to observe which reward components are higher or lower between the actions. This can provide significantly more insight into why one action is ranked as higher than another.}

Recent work showed how to learn from such decomposed reward function in a way that aims to achieve an optimal policy and produce a decomposed Q-function $Q(s,a)$, where s is a state, and a is an action selection~\cite{erwig2018explaining}.
\FIXME{AAA - Is this Erwig paper the proper one to cite?}
This function outputs a vector for each state-action, where the $i$'th component $Q_i(s,a)$ of the Q-vector gives the expected \emph{future} total reward for the $i$'th reward component.
These decomposed reward functions make it possible to compare the Q-vectors for 2 actions and observe which reward components are higher/lower between the actions.
This provides significantly more insight into how actions are ranked.

Our work differs from~\cite{van2017hybrid} and~\cite{russell2003q}'s work because they used reward decomposition to speed up how quickly their network learned to solve problems, but we use the method as an explanation to end-users.
\cite{erwig2018explaining}'s work uses the same approach to decomposed reward bars, but our work differs through using them as an explanation to non-ML participants.
\FIXME{AAA - Don't like this. If they're interested, they can read the paper.\\They deviated from traditional reinforcement learning by running multiple off-policy algorithms in parallel, each optimizing their own value functions (the ``decomposition" in this case).}
%Our work differs because we are less focused on how this method can be used to optimize a network and more on how it can be used as an explanation for end-users.


%Russell et al. used reinforcement learning with problems that had subtasks, using multiple agents working in concert to solve them~\cite{russell2003q}.
%\FIXME{This paper is primarily concerned with training an agent by first training a bunch of ``subagents" on smaller tasks or ``subgoals".
%This notably deviates from our approach both in that we aim to use the decomposition purely for explanation purposes, and we aim to estimate a single overall value function in a game without explicit subgoals.}
%They were concerned with training an agent through training a set of ``subagents'' on smaller tasks (``subgoals'').
%Our approach differs because we aim to use the decomposition purely for explanation purpose and estimate a single value function without explicit subgoals.

%Our work also differs from Erwig et al.'s, since they used a minimally sufficient explanation to explain a deep network, whereas we don't omit any of the decomposed reward bars and study in a controlled lab setting.
%Erwig et al. investigated how to to use a similar decomposed reward method to explain a deep network using a minimally sufficient explanation~\cite{erwig2018explaining}.
%Our work differs because we do not use their minimally sufficient explanation, wanting to investigate if people can understand the decomposed rewards before any data is removed from the user.
%This was an attempt to have our explanations be as complete as possible.
%Our work also differs because we used users in a lab to gauge the effectiveness of the decomposed reward bars





\subsubsection{How do we define an explanation}

\boldify{We define an explanation as a tuple Explanation = < Artifact, Behaviors, Score>, where Artifacts $\in$ \{Saliency, Rewards, Saliency + Rewards\}, Behaviors are considered the feedback received from clicking on any of the above, and score is the displayed point value to the left of the game map. }

$Explanation \rightarrow$ $<Artifacts, Behaviors, Score>$.
Artifacts are anything displayed to assist the participant in understanding the AI's behavior, the saliency maps and/or decomposed reward bars.
The Behavior is any feedback received from clicking on any artifact.
%, such as the overlay behavior in figure~\ref{**FIXME** Postage stamp sized image with the game map/overlay behavior}.
The Score is displayed beside the game map.

\FIXME{JED: I think this artifact/behavior dichotomy is made clear with the rework to the paragraph following 2 from here}



%\boldify{Figure~\ref{fig:userInterface} shows the different types of explanations that the participants saw, and Region 4 is constant across all treatments as the area that participants answered questions}

%Figure~\ref{fig:userInterface} shows an example of what we showed participants, with highlighted regions.
%The game map is in Region 1, where the AI acts out its choice.
%The saliency maps are shown in Region 2.
%Two treatments that gave saliency maps differed in their approach to showing saliency information to prevent revealing too much about the system, but their position on the interface was consistent.
%Region 3 held the decomposed reward bars and total rewards for the 4 candidate actions.
%The legend (upper right) used color to associate a reward bar with the type of reward it represented, including the gray bars for the sum total reward bars.
%The wording was chosen to reinforce that these were predicted scores, not the actual score that the AI would receive.
%Region 4 was where questions would be posed to all participants and where they could type their responses.
%here were 4 treatments: \treatment{Control}, \treatment{Saliency}, \treatment{Rewards}, and \treatment{Everything}.

%\subsubsection{Control}

%\boldify{Region 1 in Figure~\ref{fig:userInterface} is the only region that the \treatment{Control} group saw. In their case, the explanation given to them was the game map being played, representative of how AI in RTS is handled currently}

%The \treatment{Control} participants only saw the game map in Region 1.
%No explanations were offered beyond what was visible in the game action, though the participants were free to rewind and re-watch any decision point.
%The ability to rewind and watch decision points repeatedly is how current AI systems in this domain explain themselves.

%\subsubsection{Saliency}

%\boldify{The saliency treatment had access to regions 1 \& 2. However, Figure~\ref{FIXME- Need an example} shows the type of saliency that this treatment had access to.}

%The \treatment{Saliency} participants saw both the game map and saliency maps.
%The saliency maps conveyed which features of objects the AI is looking at when it makes a decision, so they know which input matters most.

%\boldify{In order to avoid giving too much of the system away, we limited the participants' view of saliency to \emph{just} the action that was taken, so if the AI attacked Quadrant 1 (Q1), then we only showed the participants the saliency that was relevant to Q1.}

%The \treatment{Saliency} treatment's saliency maps express information about what the AI was focusing on \emph{only} for the action selected, so the participants learned nothing about reward bars.
%This maintained the study's integrity and abides by~\cite{kulesza2015principles}'s last principle about overwhelming.
%A more detailed approach was used in the ``Everything'' treatment, but the action-level granularity used here was chosen for 2 reasons.
%First, the more detailed approach exposes additional information about the AI's inner workings that we did not want exposed in this treatment.
%Second, showing this level of detail abides by Kulesza et al.'s last principle to not overwhelm the user~\cite{kulesza2015principles}.

%\subsubsection{Rewards}
%\boldify{Humans perform cost/benefit analysis all the time, even in the likes of their foraging behavior ~\cite{ FIXME any of the IFT work will do} }

%Humans routinely perform cost/benefit analysis, trading off between expected rewards and time investment for those rewards.
%This has been shown across a variety of domains from library card organization~\cite{pirolli1999information} to debugging tasks~\cite{piorkowski2015fix}.
%The \treatment{Rewards} treatment showed predicted costs and benefits of taking actions.

%\boldify{By phrasing the reward bars as a cost (bars below zero in Figure~\ref{fig:userInterface}, region 2)) and benefit (positive bars in that figure) prediction, we wanted to see if humans could infer these from the visual representation of \emph{why} the AI thought the way it did}

%We wanted to see if the AI's thought process, or aspects of it, could be inferred by participants, since the decomposed reward bars were framed as a cost (bars $< 0$) and benefit(bars $> 0$) analysis from the AI.
%Participants were shown both the decomposed reward bars (the thin ones) and the sum total (the gray ones) for each possible action.

%\subsubsection{Saliency, Rewards, and everything else}
%\boldify{The Saliency, Rewards, and Everything Else treatment, referred to as the ``Everything'' treatment, was a combination of the saliency maps and the reward bars, where each row of saliency corresponded with a decomposed reward bar}

%The \treatment{Everything} treatment showed the participants all the explanation detail our system could provide.
%The saliency maps corresponded to a particular predicted reward type for each action.
%For example, the top row of saliency corresponded with a bar in Attack Q1, the second row corresponded to the same bar type in Attack Q2, and so on.
%This level of detail was consistent with~\cite{kulesza2015principles}'s principle to be complete.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% JED: Old technical methodology about reward decomposition

\boldify{ Different events in the game are assigned a component or type based on their source and context. 
For instance, taking damage from an enemy may yield a small negative reward named "Took Damage" equal to the damage taken. 
This allows us to narrow down what sort of action the agent may have been seeking out or avoiding in a given decision.}

Reward decomposition bars assign context and types to different events, making an environment's total reward.
Our AI learned a positive/negative reward for damaging objects, and it also learned a destruction bonus/penalty, depending on if it's a friend or an enemy.
For example, if it hurts a friendly object, it loses 10 points for damage, but if it hurts an enemy, it gains 10 points for damaging it.

\boldify{
(NB could mention we use experience replay and dual networks).}

We trained a SARSA network to predict Q-values for these rewards, such that the sum of the reward types was the total reward ($\epsilon$-Q-values) for each action.
All of this information was presented to the participants as an explanation.

%We displayed these values as explanations to the user via a bar chart, showing the relative values for each action at a given decision. 
%We also have ``total" bars behind each group to communicate to the user what the total predicted Q value was, as that's the value used to make the decision.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AAA: The ``Everything is needed when hard'' section










Businesses like DeepMind have only recently made a ``good'' AI for StarCraft II, which has beaten 2 professionals that could play at the top 1\% of all human players.
However, with an action space of $10^{26}$ possible moves, it would be difficult to assess the effectiveness of these visual explanations.
By reducing the action space to 4 possible moves, the participants were more likely to focus on the explanations, rather than on the game action.









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%AAA: Moved this from the end of methodology (technical methodology)


\FIXME{JED @ AS: If what I wrote above here looks good, I will move everything below here to leftovers}
-------------------------------------

-------------------------------------

-------------------------------------

-------------------------------------



\FIXME{ OLD VERSION AAA - Starting with the HP, we perturbed the HP of each object, noted the output for each output class and reward type, and subtracted that from the corresponding original un-perturbed image output. We noted this difference and inserted this value in the corresponding object's pixels in the HP Saliency Map for the corresponding output class and reward type. 
Similarly, the enemy tank if present, was perturbed, and the difference between the perturbed image output and the unperturbed image output was inserted into the coordinates of the tank in the tank saliency map. }

Hp was real-valued, whereas all others were binary (there or not there), so we perturbed the HP of each object for each reward type and output class and subtracted that from the original un-perturbed image output.
This difference was inserted into each object's pixel coordinates in the corresponding saliency map.
Enemy tanks had a similar approach, but only switching between $1 \leftrightarrow 0$ in the layer.



For Size, each object on the map had its pixels zeroed out and turned to 1 in its opposing size layer.
Thus, a small fort in top-right quadrant would have its pixels zeroed out in the \textbf{small} fort layer.
Its pixels would then turn to 1 in the \textbf{big} forts layer.
These transformations changed $Small forts\leftrightarrow Big forts$ and $towns \leftrightarrow cities$.
An identical approach was taken for the City/Fort layer, where the transformations were $Forts \leftrightarrow Town/City$, depending on the size of the Fort.


\FIXME{OLD VERSION AAA - The Friend/Enemy saliency map has the same approach as the previous two except here we switched the pixel coordinates of objects between the friend and enemy objects and layers. }

The Friend/Enemy layer's transformations changed between $Friend \leftrightarrow Enemy$, except the pixel coordinates of objects switched between friend/enemy objects and layers.

\boldify{For the output, we combined some of the maps together, and we did this because....}
\FIXME{OLD VERSION AAA - The output saliency reflects five of the most pressing factors that would impact a neural network's decision. 
The saliency values are highly skewed, with the friend/enemy map usually having the highest values, thus being the most important to the network. 
It was a challenge, therefore, to choose an apt normalization method. 
We decided to globally normalize the saliency values. 
We ran the agent for 16000 episodes, and chose the maximum value for each map for each reward type and output class. 
We then used these values to normalize the respective map for that reward type and output class.}

In order to accurately reflect the AI's internal reasoning, we found a global normalization value for \emph{each} reward type and output class of attacking a quadrant by running 16000 episodes and choosing the max value for each saliency map.
We then normalized the 5 maps that reflect the most pressing factors impacting the network's decision.
This put every pixel's value $\in [0,1]$.
We took these values and colored them between [black, white].
As the pixels became more yellow, and eventually white, the more important they were.
These maps were presented to the participants of the \treatment{Saliency} and the \treatment{Everything} treatments, and the visualization was chosen to be consistent with prior research~\cite{newn2017evaluating}.





%------------------------------------------------------------
%AAA: Tanks don't matter


\subsection{What did participants learn over time?}


\boldify{We know they didn't learn much overall; look how varying the data is, but one concept shines through}

As Figure~\ref{fig:predictiveAccuracy} clearly shows, none of the treatments tended to improve over time, which is consistent with the possibility raised in Section **4.3** that different situations (here, different decision points) may require different kinds of things explained.
However, there was one notable exception -- participants who saw rewards \treatment{Rewards} + \treatment{Everything} seemed to get better at sorting out which game objects \emph{don't} matter to the AI.




\boldify{For example, look at Figure~\ref{fig:learnedConcepts}. The people that saw rewards always do better}

Figure~\ref{fig:learnedConcepts} shows that at all DPs with enemy tanks, the \treatment{Rewards} + \treatment{Everything} group slightly outperformed the others.
For example, at DP7, 52\% of these combined groups predicted correctly that the AI would \emph{not} attack the tank, opposed to 37\% of the other combined groups.
At this decision, 2 participants predicted: ``\textit{I think the value for destroying the enemy fort will be larger than ... preserving the friendly city...}''\user{R}{21}{10191201} and ``\textit{according to previous saliency map tank will choose [the enemy tank] for sure because its attention in every aspect was toward this object.}''\user{S}{31}{10121805}.
Two conclusions using the explanations, but only one was right.

%\boldify{The benefit of reward bars for prediction is that they can reveal these concepts}





\boldify{We might expect that there's a learning effect as time goes on, but our data shows that they don't with peaks and valleys. What do they learn? Tanks don't matter!}

\input{figure/learnedConcepts.tex}
However, there are concepts that \emph{some} participants learned from certain situations, such as when enemy tanks are present (DP3, DP4, \& DP7).
%The participants in \treatment{Everything} \& \treatment{Rewards} caught on to.
Figure~\ref{fig:learnedConcepts} shows that at all three of these points, the combined \treatment{Rewards} + \treatment{Everything} participants had slightly higher predictive accuracy.

\boldify{DP3 is easy, so everyone gets it right, but DP4 saw a sharp decline; here are some quotes that give us insights.}

DP3 was ``easy'' for everyone, as 89\% of participants correctly predicted the action, since this map only had one enemy: the enemy tank (Table~\ref{table:DecisionPoints}). 


% C = 81, S = 90, R = 94, E = 90



\boldify{At DP7, those that saw rewards performed best. In fact, they performed best and for the right reasons, unlike the others.}

At DP7 (Table~\ref{table:DecisionPoints}), 52\% of participants who saw rewards (\treatment{Rewards} + \treatment{Everything}) correctly predicted that the AI attacked Q2, but only 37\% of the others guessed the same.
Some of those that did not see rewards believed the AI would protect its ally in Q1, such as: ``\textit{according to previous saliency map tank will choose [the enemy tank] for sure because its attention in every aspect was toward this object.}''\user{S}{31}{10121805}.
However, some of those that saw the bars predicted Q2 by tying what they had seen from the bars: ``\textit{I think the value for destroying the enemy fort will be larger than the value for preserving the friendly city...}''\user{R}{21}{10191201}.

When the session was nearing its end, some participants bemoaned the lack of concern the AI had for enemy tanks, such as: ``\emph{Also the reward bar does not include points for destroying an enemy tank.}''\user{R}{46}{10091203}

%\FIXME{AAA - This is the last instance of enemy tanks. I'm hoping to say that with the previous 2 decision points, this is their last opportunity to prove they've learned something, and those that saw rewards seem to have almost passed the test.}


\FIXME{AS @ : The agent behaves weirdly at the last decision point, so it will never be in line with a human's logic. Suicidal behaviour\\
AAA @ AS: I generally agree with this, but I don't think we want our readers to be questioning our AI. We can't take the risk to point at our own AI and say ``ah, it behaved weirdly. No wonder the participants couldn't predict it.''. I'll defer to MMB on this though.\\
JED: Remember that participant responses characterized the agent as behaving ``randomly''.
Thus, WHATEVER the reason the AI had for that decision, it was not known to the participants, leading them to consider it a \emph{very jarring} random choice, because it is unexpected behavior. 
This concept is important I think, because we have been consistently running into the issue of how to explain why the maximal action was taken in the presence of \textbf{action equivalency}.\\
Specifically, my thought is that the explanation consumer NEEDS to know that there is a set of actions which are all roughly interchangeable, and thus not be \emph{surprised} when any item in that set is chosen.\\
(Aside: my guess is that advantage-based views will confuse this issue by amplifying meaningless differences.
Imagine an AI choosing between US federal budget plans and returning an explanation like ``chose plan A because it saves \$1'' instead of ``these plans are interchangeable'', because that \$1 is a drop in the bucket of a trillion dollar operation.)\\
AAA: I looked back at the differences. The only one I could buy this argumentation for is D11. The AI isn't behaving randomly at any of the other 3.
%AAA: I don't even know anymore because this agent is rogue and insane. The agent wants to preserve its allies so it won't attack its friendly city in Q4. But it also wants to extend the life of the tank, and the tank might die if it attacks any enemies this turn. I would guess that the tank will attack one of the small forts in Q1 or Q2. I would attack the fort in Q2 because it has the lowest HP left. (10171805) Note: they got it right DP11
%\\AAA: There are two enemy forts on the map, one that is small and barely damaged, and one that has already had some damage done to it. Thus I think the agent would combine the friend/enemy saliency map with the HP map and maybe with the size map too to decide to attack the enemy fort in Q2. (10171805) DP8

%
%
%This paper provides a framework for human-subject studies to evaluate XAI systems, illuminating a path forward for those struggling with similarly noisy prediction data.
%However, explanation for AI is still ongoing research;
%they raise questions like: ``\emph{How are you making `smart' decisions right now with semi-flawed reasoning? I don't understand!}''\user{S}{87}{10171805}


%\FIXME{Participant quotes we might use for sunset
%
%(helpful/problematic data)
%At first, I was a little confused by the saliency maps. I %understand what they were meant to be, but it took me a while %to fully integrate the saliency maps into my thought process.
%
%There would be points when I didn’t understand why the AI %valued one object more than the other based of the saliency %maps.
%
%(lim-dey)
%How are you making "smart" decisions right now with semi-flawed reasoning? I don't understand!
%
%(Not sure what data source)
%Going for the big fort with the most HP when you are at 1/8th %of your max HP seems like an unwise decision. Perhaps the AI %decides to go all out when faced with an option when the tank %will almost certainly die when it engages.
%}


\mysubsubsection{The last decision is coming}


%\input{figure/endOfTask.tex}

\boldify{The third flavor of decision point are those that end a task, where we have discussed previously that those that saw saliency perceive that the AI behaves differently}

DP4, DP8, DP11, and DP14 were all final decision points of a task, when the ``Episode [was] Over'' (Table~\ref{table:MentalModelCodes}).
We highlight two of these, DP8 and DP14, where the \treatment{Saliency} treatment performed significantly better than the others, aligning with the result that those with saliency noticed situational differences (Figure~\ref{fig:predictiveAccuracy}).

\boldify{At DP8, the participants who saw \emph{just} saliency performed much better than the participants that saw \emph{just} rewards.}

At DP8 (Table~\ref{table:DecisionPoints}), 87 participants (70\%) guessed correctly that Q2 was the AI's choice, but 16 participants in the \treatment{Rewards} treatment (50\%) were incorrect.
Some of the \treatment{Saliency} participants correctly deduced why the AI would attack here, such as: ``\textit{The agent has shown that it prioritizes bases and sizes when making decisions.}''\user{S}{122}{10121201}.
However, some of the participants in the \treatment{Rewards} treatment struggled, such as this participant that selected Q3: ``\textit{Due to low tank health it cannot destroy either of the enemy forts. So going to the smaller fort might give more damage rewards.}''\user{R}{70}{9301201}.
%83.6\% correct for those that saw saliency maps
%58.7\% correct for those that didn't.

\boldify{At DP14, the saliency really leads, performing well compared to the same aforementioned treatments}

At DP14 (Table~\ref{table:DecisionPoints}), Q2 \& Q4 had low health, but Q3 had $\approx 75\%$ health.
The \treatment{Saliency} treatment was the only one to get above 33\% accuracy that the AI would attack Q3.
Some of the successful participants in this treatment relied on gathered knowledge, for example: ``\emph{The agent has been focusing on high health Large Forts}''\user{S}{25}{9291210}.
However, some in the other treatments show a deference to the current board state, like \user{R}{40}{10201205} that selected Q4 ``\textit{the fort is an enemy and it has the lowest health points among the enemies on the board}''.

\boldify{With the exception of DP4, the treatments that see rewards never perform the best. This means there's something distracting about the decomposed reward bars closer to the end of a task. However, what makes DP4 special?}

%As the participants progress, they gather knowledge to apply to each prediction.
%However, towards the end of a task, the reward bars get much smaller and harder to interpret.
%As they try to tie together different pieces of information from the past, it can confuse the participants and overwhelm them.

%DP 8, $p$ = 0.0114, DP 14 $p$ = 0.0252

==> b-leftovers.tex <==
%\fakeResult{We have two areas of interest from this graph. 1) When there are massive dips (Decision points 4, 7, 10, 12, 14), what's causing them? 2) Since saliency performs best overall (5 instances out of 14 decision points), why are they performing the best?}
%GLOBAL TO DO: avoid words like better or worse unless we have the statistical information to back it up, since most of the reviewers are statistically minded.

%\fakeResult{to answer 1), we first looked at the situations that the AI found itself in. These can be classified in two types:\\ a) ``Help my friends!'' (Decisions 4, 7)\\b)``It sure is a close call...'' (Decisions 10, 12, 14)\\FIXME - Put in some visualisation for this.}
%Put the maps in, postage stamp size. All they need to see is ``look, no friends!''

%About point (a) above, Russell \&....
%\fakeResult{Russell \& Norvig speak about 2 types of thoughts/behaviors for AI: Acting Humanly and Acting Rationally. When an AI behaves humanly, it solves problems the same way that a human does and acts the way that the human will, the Turing Test approach. When an AI behaves rationally, it seeks to maximize the expected value of its performance measure.}

%\fakeResult{In the instance of ``Help my friends!'', Participants desired for the artificial intelligence to save a town/city that couldn't fight back against the black enemy tank. They cited the current state of the map and gave us reasoning that followed along the lines of ``The city can't fight back, so it should save its friends''}

%\fakeResult{However, the AI believed that it could end the episode before its friend died or took too much damage, or it simply was going to gain more points by attacking another object.}

%We have no data about the future, so don't say will correct. We can say did correct if we have the data to back it up. No preesnt tense in results, no future tense in results. Can use present tense in the likes of definitions.
%\fakeResult{This is an example where the participants' expectation for the AI to act humanly was not met, and interestingly enough, no amount of explanation of previous behavior will correct the human thinking.}

%\fakeResult{After all, decision point 4 revealed that the AI does not protect its friends, but in a similar situation such as decision point 7, the participants still chose the enemy tank and cited similar reasoning to that of decision point 4.}

%\fakeResult{For ``It's a close call'' situations (Decisions 10, 12, 14), the participants have to decide between a variety of similar objects, where the health points of all objects are pretty close (in some instances, the difference is about 1 point)}
%Always keep in mind what the reader might want to know next, and organise around that.


\boldify{We didn't want to just collect information about \emph{what} the participants did for quantitative data, but we also wanted to know the qualitative \emph{why} of the participants}

%\FIXME{OLD VERSION AAA - Our experiment design revolved around understanding not only what the participants did for quantitative information but also the qualitative information of \emph{why} they did what they did.
%For every interaction that we asked them to perform, we also asked them to justify it in order to better understand their interactions.}

%Our experiment design was to gather information about what the participants did and qualitative information about why they did any action or thought a certain way.
%We piloted the study to try to get the highest quality of data that we could.
\FIXME{AAA @ MMB - Should we even tell them this? We don't report on the why in this paper.\\
MMB: no-- I commented it out}
\FIXME{I want this paragraph to justify the experiment design, not just reveal what the experiment design was.}

\FIXME{OLD VERSION AAA - Reward decompositions are a way to assign context and types to different events that make up an environment's total reward.
For instance, in Atari you could imagine a different reward for destroying the UFO versus destroying a normal enemy. 

In our case, we split the reward into several types based on the agent's actions: "Enemy Damaged", "Enemy Destroyed", "City Damage", "City Destroyed", "Friend Damaged", and "Friend Destroyed". 
The only positive ones are the first two, while the ones involving "City" and "Friend" (aka friendly forts) are both negative and vary only in severity. 
Rewards of differing severity need not be different types, but in this case they were semantically meaningful.}

\FIXME{OLD VERSION AAA - For Size, for each object on the map, we zeroed out the pixels and turned its pixels to 1 in its contrasting size layer.
For example, for a small fort in the top right quadrant, we zero out its pixels in the small forts layer, and turn the pixels of its coordinates to 1 in the big forts layer. 
We toggled between small and big forts, and towns and cities.
Our approach to the City/Fort is similar to the Size saliency map except we toggled between the types. So small forts and towns were switched, and big forts and cities were switched. }

==> figure/HardPoints.tex <==
\begin{figure}
	\centering
    \includegraphics[width=\linewidth]{assets/whenItsHard.png}

	
	\caption{A graph of the 2 hardest DPs. Even though the \treatment{Everything} participants do best, they aren't really doing better than random guesses.}

    
    \label{fig:HardPoints}
\end{figure}

==> figure/Overwhelm.tex <==
\begin{figure}
	\centering
    \includegraphics[width=\linewidth]{assets/Overwhelm.png}

	
	\caption{A graph of all treatments' accuracy when the ``Episode [was] Over''. Notice that twice, the \treatment{Saliency} participants performed best twice.}

    
    \label{fig:Overwhelm}
\end{figure}

==> figure/Prediction_1_.tex <==
\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{assets/Prediction(1)}
	\caption{
    An example of the interface as the control sees it.
}
	\label{fig:controlInterface}

\end{figure}

==> figure/learnedConcepts.tex <==
\begin{figure}
	\centering
    \includegraphics[width=\linewidth]{assets/TanksDoNotMatter.pdf}

	
	\caption{A graph of all treatments' accuracy for maps that had enemy tanks. Those who did not see rewards (%
	\colorboxBackgroundForegroundText{ControlColor}{white}{Control}
	+
	\colorboxBackgroundForegroundText{SaliencyColor}{black}{Saliency}%
	) had lower predictive accuracy at all of these points than those who did see rewards (%
	\colorboxBackgroundForegroundText{RewardsColor}{black}{Rewards}
	+ 
	\colorboxBackgroundForegroundText{EverythingColor}{white}{Everything}%
	).}

    
    \label{fig:learnedConcepts}
\end{figure}

==> figure/noExplanation.tex <==
\begin{figure}
	\centering
    \includegraphics[width=\linewidth]{assets/noExplanationRequired.png}

	
	\caption{A graph of all treatments' accuracy at DP2, DP5, and DP13. 
	In some cases, the \treatment{Control} treatment may perform well enough without an explanation.}

    
    \label{fig:noExplanations}
\end{figure}

==> figure/sawRewards.tex <==
\begin{figure}
	\centering
	\includegraphics[width = \linewidth]{assets/sawRewards.png}
	\caption{The mental model scores for those that saw decomposed reward bars and those that did not.
	\treatment{SawRewards} performed much better than \treatment{DidNot}.}
	\label{fig:sawRewards}

\end{figure}

==> figure/sawSaliency.tex <==
\begin{figure}
	\centering
	\includegraphics[width = \linewidth]{assets/sawSaliency.png}
	\caption{The mental model scores for those that saw saliency maps and those that did not. \treatment{SawSaliency} performed marginally better than \treatment{DidNot}.}
	\label{fig:sawSaliency}

\end{figure}

==> tables/questionTable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{5}{|c|}{\textbf{Questions asked by treatment}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
   & Control                                                                                                                                                                                & Saliency                                                                                                                                                                                          & Rewards                                                                                                                                                                  & Everything                                                                                                                                                                                             \\ \hline
Q1 & \multicolumn{4}{l|}{\begin{tabular}[c]{@{}l@{}}On the game map (above), which object do you think the AI will send the tank to attack?\\ Please click on that object\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \hline
Q2 & \multicolumn{4}{l|}{\begin{tabular}[c]{@{}l@{}}Why do you think the AI would attack this object? (A few sentences, as detailed as\\ possible)\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
Q3 & \begin{tabular}[c]{@{}l@{}}After playing this\\ decision, click on\\ the object on the\\ game map (above)\\ that you think the\\ AI was paying\\ the most attention\\ to.\end{tabular} & \begin{tabular}[c]{@{}l@{}}After playing this\\ decision, which\\ saliency map (below)\\ do you think was the\\ most influential in\\ this decision? (Please\\ click on exactly one)\end{tabular} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}After playing this decision point, which\\ reward bar (right) do you think influenced\\ the agent's decision the most? (Please\\ click on it).\end{tabular}}                                                                                                                                                                       \\ \hline
Q4 & \begin{tabular}[c]{@{}l@{}}For what reason(s)\\ would the AI pay\\ attention to this\\ object? (A few\\ sentences, as\\ detailed as possible)\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}Why was the map you\\ selected the most\\ influential to the agent?\\ (A few sentences, as\\ detailed as possible).\end{tabular}                                       & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Why did the bar you selected matter the\\ most to the agent? (A few sentences, as\\ detailed as possible).\end{tabular}}                                                                                                                                                                                                           \\ \hline
Q5 & \begin{tabular}[c]{@{}l@{}}Do you think there is\\ a flaw in the AI's\\ reasoning? If so, what\\ is that flaw?\end{tabular}                                                            & \begin{tabular}[c]{@{}l@{}}From looking at the\\ saliency maps (below),\\ do you think there is a\\ flaw in the AI's\\ reasoning? If so, what\\ is that flaw?\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}From looking at the\\ reward bars (right),\\ do you think there is a\\ flaw in the AI's\\ reasoning? If so, what\\ is that flaw?\end{tabular} & \begin{tabular}[c]{@{}l@{}}Which saliency map (below)\\ do you think was the most\\ influential in this decision?\\ (Please click on exactly one)\end{tabular}                                         \\ \hline
Q6 & \multicolumn{3}{c|}{\multirow{2}{*}{N/A}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}Why was the map you\\ selected the most influential\\ to the agent? (A few\\ sentences, as detailed as\\ possible).\end{tabular}                                            \\ \cline{1-1} \cline{5-5} 
Q7 & \multicolumn{3}{c|}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}From looking at the saliency\\ maps (below) and the\\ reward bars (right), do you\\ think there is a flaw in the\\ AI's reasoning? If so, what\\ is that flaw?\end{tabular} \\ \hline
Q8 & \multicolumn{4}{l|}{What, if anything, do you want to ask the AI at this point?}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \hline
\end{tabular}
\caption{All the questions asked to the participants.}

\label{table:questionsAsked}

\end{table}
